Electrolyzer Scheduling for Nordic FCR Services

The cost competitiveness of green hydrogen production via electrolysis presents a significant challenge for its large-scale adoption. One potential solution to make electrolyzers profitable is to diversify their products and participate in various markets, generating additional revenue streams. Electrolyzers can be utilized as flexible loads and participate in various frequency-supporting ancillary service markets by adjusting their operating set points. This paper develops a mixed-integer linear model, deriving an optimal scheduling strategy for an electrolyzer providing Frequency Containment Reserve (FCR) services in the Nordic synchronous region. Depending on the hydrogen price and demand, results show that the provision of various FCR services, particularly those for critical frequency conditions (FCR-D), could significantly increase the profit of the electrolyzer.

==> Sections/figure_old.tex <==
\begin{figure}[]
\centering


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Rounded Rect [id:dp4332644849152041] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.11 ] (51.64,101.75) .. controls (51.64,96.74) and (55.7,92.69) .. (60.7,92.69) -- (95.94,92.69) .. controls (100.94,92.69) and (105,96.74) .. (105,101.75) -- (105,128.94) .. controls (105,133.94) and (100.94,138) .. (95.94,138) -- (60.7,138) .. controls (55.7,138) and (51.64,133.94) .. (51.64,128.94) -- cycle ;
%Straight Lines [id:da6394219194815551] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.11 ]   (106.14,116.69) -- (165.14,116.69) ;
\draw [shift={(167.14,116.69)}, rotate = 180] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp1610231766721204] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.11 ] (167.14,101.25) .. controls (167.14,96.24) and (171.2,92.19) .. (176.2,92.19) -- (220.44,92.19) .. controls (225.44,92.19) and (229.5,96.24) .. (229.5,101.25) -- (229.5,128.44) .. controls (229.5,133.44) and (225.44,137.5) .. (220.44,137.5) -- (176.2,137.5) .. controls (171.2,137.5) and (167.14,133.44) .. (167.14,128.44) -- cycle ;
%Straight Lines [id:da4063914392785488] 
\draw [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ]   (229.17,116.17) -- (264.14,116.19) ;
\draw [shift={(266.14,116.19)}, rotate = 180.03] [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Manual Operation [id:dp06081476023702681] 
\draw  [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ] (306.5,130.4) -- (266.5,138.69) -- (266.5,94.5) -- (306.5,102.79) -- cycle ;
%Straight Lines [id:da9049840103715661] 
\draw [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ]   (306.64,118.19) -- (335.16,92.53) ;
\draw [shift={(336.64,91.19)}, rotate = 138.01] [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Magnetic Disk [id:dp9058486737716807] 
\draw  [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ] (386.32,71) -- (386.32,98.18) .. controls (386.32,102.22) and (375.24,105.5) .. (361.57,105.5) .. controls (347.9,105.5) and (336.82,102.22) .. (336.82,98.18) -- (336.82,71)(386.32,71) .. controls (386.32,75.05) and (375.24,78.32) .. (361.57,78.32) .. controls (347.9,78.32) and (336.82,75.05) .. (336.82,71) .. controls (336.82,66.96) and (347.9,63.69) .. (361.57,63.69) .. controls (375.24,63.69) and (386.32,66.96) .. (386.32,71) -- cycle ;
%Rounded Rect [id:dp26633183021676565] 
\draw  [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ] (335.43,136.89) .. controls (335.43,134.02) and (337.76,131.69) .. (340.63,131.69) -- (388.37,131.69) .. controls (391.24,131.69) and (393.57,134.02) .. (393.57,136.89) -- (393.57,152.49) .. controls (393.57,155.36) and (391.24,157.69) .. (388.37,157.69) -- (340.63,157.69) .. controls (337.76,157.69) and (335.43,155.36) .. (335.43,152.49) -- cycle ;
%Straight Lines [id:da2361102252268057] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=0.1 ]   (198.64,92.69) -- (198.64,68.69) ;
\draw [shift={(198.64,66.69)}, rotate = 90] [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp12189549280437273] 
\draw  [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=0.1 ] (163.5,50.25) .. controls (163.5,48.01) and (165.32,46.19) .. (167.56,46.19) -- (229.44,46.19) .. controls (231.68,46.19) and (233.5,48.01) .. (233.5,50.25) -- (233.5,62.44) .. controls (233.5,64.68) and (231.68,66.5) .. (229.44,66.5) -- (167.56,66.5) .. controls (165.32,66.5) and (163.5,64.68) .. (163.5,62.44) -- cycle ;
%Straight Lines [id:da4669227648468448] 
\draw [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ]   (306.64,118.19) -- (333.66,142.84) ;
\draw [shift={(335.14,144.19)}, rotate = 222.37] [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da055810511223996606] 
\draw [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ]   (361.57,105.5) -- (362.1,129.69) ;
\draw [shift={(362.14,131.69)}, rotate = 268.75] [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp18634032002229772] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.05 ] (47.5,40.5) .. controls (47.5,36.08) and (51.08,32.5) .. (55.5,32.5) -- (135.5,32.5) .. controls (139.92,32.5) and (143.5,36.08) .. (143.5,40.5) -- (143.5,64.5) .. controls (143.5,68.92) and (139.92,72.5) .. (135.5,72.5) -- (55.5,72.5) .. controls (51.08,72.5) and (47.5,68.92) .. (47.5,64.5) -- cycle ;
%Rounded Rect [id:dp46167155507627844] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.11 ] (52.99,37.83) .. controls (52.99,36.85) and (53.79,36.05) .. (54.77,36.05) -- (60.72,36.05) .. controls (61.7,36.05) and (62.5,36.85) .. (62.5,37.83) -- (62.5,43.17) .. controls (62.5,44.15) and (61.7,44.95) .. (60.72,44.95) -- (54.77,44.95) .. controls (53.79,44.95) and (52.99,44.15) .. (52.99,43.17) -- cycle ;
%Rounded Rect [id:dp4802170058126627] 
\draw  [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=0.1 ] (52.99,50.21) .. controls (52.99,49.19) and (53.82,48.36) .. (54.85,48.36) -- (60.51,48.36) .. controls (61.54,48.36) and (62.37,49.19) .. (62.37,50.21) -- (62.37,55.79) .. controls (62.37,56.81) and (61.54,57.64) .. (60.51,57.64) -- (54.85,57.64) .. controls (53.82,57.64) and (52.99,56.81) .. (52.99,55.79) -- cycle ;
%Rounded Rect [id:dp8229632552801993] 
\draw  [color={rgb, 255:red, 80; green, 227; blue, 194 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.07 ] (52.64,61.83) .. controls (52.64,60.85) and (53.44,60.05) .. (54.42,60.05) -- (60.37,60.05) .. controls (61.35,60.05) and (62.15,60.85) .. (62.15,61.83) -- (62.15,67.17) .. controls (62.15,68.15) and (61.35,68.95) .. (60.37,68.95) -- (54.42,68.95) .. controls (53.44,68.95) and (52.64,68.15) .. (52.64,67.17) -- cycle ;

% Text Node
\draw (170.82,102.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{39.23pt}\setlength\topsep{0pt}
\begin{center}
Alkaline\\electrolyzer
\end{center}

\end{minipage}};
% Text Node
\draw (166,50.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{45.57pt}\setlength\topsep{0pt}
\begin{center}
FCR services
\end{center}

\end{minipage}};
% Text Node
\draw (268,105.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{24.15pt}\setlength\topsep{0pt}
\begin{center}
\ce{H2} \\compr.
\end{center}

\end{minipage}};
% Text Node
\draw (343,79) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{26.54pt}\setlength\topsep{0pt}
\begin{center}
\ce{H2} \\storage
\end{center}

\end{minipage}};
% Text Node
\draw (336.5,139.89) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{39.64pt}\setlength\topsep{0pt}
\begin{center}
\ce{H2} demand
\end{center}

\end{minipage}};
% Text Node
\draw (65.5,35.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Grid operations};
% Text Node
\draw (65.5,48) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {FCR operations};
% Text Node
\draw (65.5,59.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\ce{H2} operations};
% Text Node
\draw (61.32,102.84) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{24.95pt}\setlength\topsep{0pt}
\begin{center}
Power \\grid
\end{center}

\end{minipage}};
% Text Node
\draw (107.32,89.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{34.86pt}\setlength\topsep{0pt}
\begin{center}
TSO/DSO\\tariff
\end{center}

\end{minipage}};


\end{tikzpicture}

\caption{Power system design of an alkaline electrolyzer  and auxiliary assets, providing hydrogen and ancillary services. The power source is the grid.}
\label{fig:power_diagram}
\figspace
\end{figure}
